VILA: On Pre-training for Visual Language Models

Visual language models (VLMs) rapidly progressed with the recent success of large language models. There have been growing efforts on visual instruction tuning to extend the LLM with visual inputs, but lacks an in-depth study of the visual language pre-training process, where the model learns to perform joint modeling on both modalities. In this work, we examine the design options for VLM pre-training by augmenting LLM towards VLM through step-by-step controllable comparisons. We introduce three main findings: (1) freezing LLMs during pre-training can achieve decent zero-shot performance, but lack in-context learning capability, which requires unfreezing the LLM; (2) interleaved pre-training data is beneficial whereas image-text pairs alone are not optimal; (3) re-blending text-only instruction data to image-text data during instruction fine-tuning not only remedies the degradation of text-only tasks, but also boosts VLM task accuracy. With an enhanced pre-training recipe we build VILA, a Visual Language model family that consistently outperforms the state-of-the-art models, e.g., LLaVA-1.5, across main benchmarks without bells and whistles. Multi-modal pre-training also helps unveil appealing properties of VILA, including multi-image reasoning, enhanced in-context learning, and better world knowledge.

==> figure_text/fig_cos_sim.tex <==
\begin{figure*}[t]
    \centering
     \includegraphics[width=0.9\textwidth]{figures/cos_sim_curve.pdf}
    \caption{Cosine similarities of visual and textual embeddings (Shamfer distance) across different blocks. \textbf{(a)} Prompt-tuning to support visual tokens can only enable shallow alignment, while fine-tuning the LLM leads to alignment at deeper layers. From configuration (b) to (d) (as in Table~\ref{tab:training_ablate}), the alignment improves at deeper layer, so as ICL accuracy (4-shot). 
    \textbf{(b)} Visual token range mapping improves the embedding alignment for the shallow layers. The  visual-textual token alignment now matches the intra-text alignment (dashed line).  
    } 
    \label{fig:cos_sim}
\end{figure*}


==> figure_text/tab_data_blend.tex <==
% \renewcommand \arraystretch{0.93}
\begin{table*}[t]
    % \setlength{\tabcolsep}{3pt}
    \small
    \centering
    \begin{tabular}{lccccl}
        \toprule
        & \multicolumn{2}{c}{Data Type} &  \multicolumn{2}{c}{VLM acc (avg)} &  \multirow{2}{*}{MMLU acc}    \\ \cmidrule(lr){2-3}  \cmidrule(lr){4-5}  
        & PT & SFT &  0-shot & 4-shot  \\ \midrule
        \rowcolor{black!10}
         \emph{Llama-2} & - & - & - & - & \emph{46.0\%} \\ 
         % & -  &  Text & - & - & 51.2\% \\\midrule
         % llama2-7b-coyo-finetune-cleanflannosys+llava-linear-e1-nose-run2
        (i) & COYO & Visual &  51.1\% & 50.3\%  & 28.8\% (\textcolor{mydarkred}{-17.2\%}) \\
        % llama2-7b-mmc4sub-finetune-cleanflannosys+llava-linear-e1-nose-run2
        (ii) & MMC4 & Visual & 68.7\% & 70.9\%   & 40.7\%  (-5.3\%) \\ \midrule
        % llama2-7b-mmc4sub+coyo-finetune-cleanflannosys+llava-linear-e1-nose-run2
        (iii) & MMC4+COYO & Visual  & 68.7\% & 71.3\% & 40.2\% (-5.8\%) \\ \midrule 
        \rowcolor{black!10}
        \emph{Llama-2} & - & \emph{Text} & - & - & \emph{51.2\%} \\  
        % llama2-7b-mmc4sub-finetune-cleandualflan+llava+sgpt-linear-e1-nose-run2
        (iii) & MMC4 & Vis.+Text  & 71.0\% & 72.1\% & 51.4\% (\textcolor{mydarkgreen}{+0.2\%}) \\
        % llama2-7b-mmc4sub+coyo-finetune-cleandualflan+llava+sgpt-linear-e1-nose-run2
        (iv) & MMC4+COYO & Vis.+Text  & \textbf{72.3\%} & \textbf{73.6\%} & 50.9\% (\textcolor{mydarkgreen}{-0.3\%})\\
        \bottomrule
    \end{tabular}
    \caption{TODO \ji{maybe remove row iii and v? to make comparison more clear}}
    \label{tab:data_blend}
\end{table*}



==> figure_text/tab_license_json.tex <==
\begin{table}
  \begin{minipage}{0.99\linewidth}
\centering
\scalebox{0.8}{
\begin{tabular}{p{1.3cm} p{8.0cm} }
\toprule
 \multicolumn{2}{l}{\bf Visual input example, Constrained JSON Output:}  \\
\midrule
&  \includegraphics[height=3.5cm]{figures/ima_cardholder.jpg} \\

\textbf{User} & Please read the text in this image and return the information in the following JSON format (note xxx is placeholder, if the information is not available in the image, put "N/A" instead). \\
& {\small \{"class": xxx, "DLN": xxx, "DOB": xxx, "Name": xxx, "Address": xxx, "EXP": xxx, "ISS": xxx, "SEX": xxx, "HGT": xxx, "WGT": xxx, "EYES": xxx, "HAIR": xxx, "DONOR": xxx\}} \\
\midrule
\textbf{GPT-4V} & {\small \{"class": "C", "DLN": "\hl{~}1234568", "DOB": "08/31/1977", "Name": "Ima Cardholder", "Address": "2570 24th Street, Anytown, CA 95818", "EXP": "08/31/2014", "ISS": "08/31/\hl{2011}", "SEX": "F", "HGT": "5-05", "WGT": "125 lbs", "EYES": "BRN", "HAIR": "BRN", "DONOR": "\hl{VETERAN}"\}} \\
% \midrule
% \shortname{} & {\small \{"class": "Driver License", "DLN": "CA123 456 789", "DOB": "01/01/1990", "Name": "Amy", "Address": "Anytown, CA", "EXP": "08/31/2023", "ISS": "Veteran", "SEX": “F", "HGT": "5'5", "WGT": "130", "EYES": "Brown", "HAIR": "Brown", "DONOR": "Unknown"\}} \\
\midrule
\textbf{LLaVA-1.5} & {\small \{"class": "C", "DLN": "\hl{1132}45678\hl{9}", "DOB": "08/\hl{23}/197\hl{1}", "Name": "Ima Cardholder", "Address": "\hl{~}Anytown, \hl{State, Zip}", "EXP": "08/\hl{23}/2014", "ISS": "\hl{California}", "SEX": "F", "HGT": "5'5", "WGT": "12\hl{3}", "EYES": "Brown", "HAIR": "Brown", "DONOR": "\hl{N/A}"\}} \\
\midrule
\textbf{Ours} & {\small \{"Class": "C", "DLN": "123456789", "DOB": "1990-08-31", "Name": "Irma Cardholder", "Address": "Anytown, CA 90000", "EXP": "08/31/2014", "ISS": "CA", "SEX": "F", "HGT": "5'4", "WGT": "120", "EYES": "Brown", "HAIR": "Black", "DONOR": "N/A"\}} \\
\bottomrule
\end{tabular}
}
% \vspace{1mm}
\captionof{table}{TODO. GPT-4V results are obtained from \cite{yang2023dawn}.}
\label{tab:constrait_json}  
  \end{minipage}
\end{table}



==> figure_text/tab_pretrain_breaks_text_only.tex <==
% \renewcommand \arraystretch{0.93}
\begin{table}[t]
    % \setlength{\tabcolsep}{3pt}
    \small
    \centering
    \begin{tabular}{lccc}
        \toprule
        &\multirow{2}{*}{\shortstack{MMLU \\Acc. $\uparrow$}} &  \multicolumn{2}{c}{MMC4 (val) PPL $\downarrow$} \\  \cmidrule(lr){3-4}
        % & MMLU acc $\uparrow$ & MMC4 ppl (w/ image) $\downarrow$& MMC4 ppl (w/o image) $\downarrow$ \\
        & & w/ image & w/o image \\ \midrule
      Original Llama-2 & \textbf{46.0\%} & - & \textbf{8.45} \\ \midrule
      Fine-tune MMC4 & 40.7\% & 9.45 & 10.09 \\
      Fine-tune COYO & \textcolor{gray!50}{28.8\%} & \textcolor{gray!50}{26.37} & \textcolor{gray!50}{115.9} \\ \midrule
      Fine-tune MMC4 \emph{VExp.} & \textbf{46.0\%}  & \textbf{8.18} & \textbf{8.45} \\
        \bottomrule
    \end{tabular}
    \caption{Fine-tuning on image-text corpus degrades text-only accuracy due to the bad text data quality (indicated by MMLU accuracy; especially with COYO). When fine-tuned on MMC4, the model is able to better predict text tokens with the help of visual information (PPL 9.45 \vs 10.09), but the absolute PPL is worse compared to the original model (8.40) due to the degradation. Freezing the base LLM and tune the extra visiual expert (denoted as \emph{VExp.}) leads to better PPL without degrading text-only capability. }
    \label{tab:pretrain_break_text}
\end{table}


